Dropping Just a Handful of Preferences Can Change Top Large Language Model Rankings

We propose a method for evaluating the robustness of widely used LLM ranking systems -- variants of a Bradley--Terry model -- to dropping a worst-case very small fraction of preference data. Our approach is computationally fast and easy to adopt. When we apply our method to matchups from popular LLM ranking platforms, including Chatbot Arena and derivatives, we find that the rankings of top-performing models can be remarkably sensitive to the removal of a small fraction of preferences; for instance, dropping just 0.003% of human preferences can change the top-ranked model on Chatbot Arena. Our robustness check identifies the specific preferences most responsible for such ranking flips, allowing for inspection of these influential preferences. We observe that the rankings derived from MT-bench preferences are notably more robust than those from Chatbot Arena, likely due to MT-bench's use of expert annotators and carefully constructed prompts. Finally, we find that neither rankings based on crowdsourced human evaluations nor those based on LLM-as-a-judge preferences are systematically more sensitive than the other.

==> arxiv_tex/eloscore.tex <==
\section{ELO Score Computation in Chatbot Arena}
\label{sec:elo-score-computation}

Chatbot Arena computes model ELO scores using the Bradley--Terry model, implemented by fitting a logistic regression. Below, we summarize their exact steps. We follow the steps provided in \href{https://colab.research.google.com/drive/1KdwokPjirkTmpO_P1WByFNFiqxWQquwH#scrollTo=mSizG3Pzglte}{Chatbot Arena Leaderboard Calculation (Bradley-Terry model)}, a notebook provided on the Hugging Face Space developed by LMArena to recreate the leaderboard.

\begin{enumerate}
    \item \textbf{Pairwise Data Aggregation.} 
    Each match consists of a pair of models (denoted \texttt{model\_a} and \texttt{model\_b}) and a recorded winner (\texttt{model\_a}, \texttt{model\_b}, or \texttt{tie}). The match results are aggregated into three pivot tables:
    \begin{itemize}
        \item Wins for \texttt{model\_a} over \texttt{model\_b}
        \item Wins for \texttt{model\_b} over \texttt{model\_a}
        \item Ties between \texttt{model\_a} and \texttt{model\_b}
    \end{itemize}

    \item \textbf{Construction of Win-Counts Matrix.} 
    A win-counts matrix is formed where each off-diagonal entry represents twice the total number of times \texttt{model\_a} wins over \texttt{model\_b} plus the number of times they tied. i.e.,
    \[
    C_{ab} = 2 \cdot \texttt{Wins}_{a \rightarrow b} + \texttt{Ties}_{a \leftrightarrow b}.
    \]
    \item \textbf{Logistic Regression Design Matrix.} 
    For each model pair (\texttt{model\_a}, \texttt{model\_b}), two rows are added into the logistic regression design matrix. 
    \begin{itemize}
        \item The first represents \texttt{model\_a} winning over model \texttt{model\_b}.
        \item The second represents \texttt{model\_b} winning over model \texttt{model\_a}.
    \end{itemize}
    
    \item \textbf{Logistic Regression Fitting.} 
    A \textit{weighted} logistic regression model without an intercept or regularization is fit using the design matrix constructed in Step 3, with rows weighted according to the Win-Counts Matrix constructed in Step 2:
    \[
    \mathbb{P}(a \; \text{beats} \; b) = \frac{1}{1 + \exp(-(\widehat{\theta}_a - \widehat{\theta}_b))},
    \]
    where $\widehat{\theta}_n$ denotes the BT score of model $n$. 
    
    Since the weights given in Win-Counts are integer counts, fitting a weighted logistic regression is the same as fitting an unweighted logistic regression on a design matrix where each row is repeated ``weight'' number of times. A sample with weight $w$ contributes the same to the log-likelihood as if you had $w$ identical rows of that sample. In practice, we implemented the weighted regression by repeating rows, in order to make sure the setup is compatible for data dropping. To construct the new \texttt{AUGMENTED\_DATASET} such that it aligns with the weighting scheme given in the Win-Counts matrix, we
        repeat each non-tie row once. For tie rows, the original dataset denotes $0$ in the \texttt{winner\_model\_a} column as a place-in (i.e., they annotate ties with \texttt{model\_a} losing to model \texttt{model\_b}) and a $1$ in the \texttt{winner\_tie} column. To make sure ties are counted symmetrically, we add in a duplicate row with \texttt{model\_b} winning over \texttt{model\_a}.

    \item \textbf{Rescaled ELO Scores.} 
    In a postprocessing step, the learned BT scores are linearly scaled and shifted (they use \(\texttt{SCALE}=400\) and \(\texttt{INIT\_RATING}=1{,}000\)) to obtain the ELO scores:
    \[
    \texttt{ELO}_n = \texttt{SCALE} \cdot \widehat{\theta}_n + \texttt{INIT\_RATING}.
    \]
    
    If a specific reference model (they use \texttt{mixtral-8x7b-instruct-v0.1}) is included, its ELO is shifted to a fixed constant (they use $1{,}114$), and all scores are adjusted accordingly.

    To adapt our data-dropping algorithm to the postprocessing step, we apply the same linear transformation to the estimated coefficients and the data-dropping approximations. That is, all influence scores are scaled by \texttt{SCALE}. Since the shift by \texttt{INIT\_RATING} is constant, it cancels in derivatives and does not affect rankings. All ELO scores, however, are offset by \texttt{INIT\_RATING} when relevant (e.g., when interpreting absolute values like $\widehat{\theta}_n$).

    \item \textbf{Final Ranking.} 
    The ELO scores are then sorted in descending order to produce the final leaderboard.
\end{enumerate}

% (X_dup, y_dup). duplicate each win row. duplicate the ties (one in favor of A, another in favor of B).
% fit logistic regression and compute the influence scores on this data set.
% transform this back into preference data space.
% take the sum of the influence functions that belong to each preference (there are two each; these will be back-to-back.)
% sort these adjacent sum IF scores. 
% remove the top \floor{alpha N} preferences that correspond to the top scores.
% refit the model without these scores (for the ties, we default to the way that they are displayed in the original data, which is always, model A loses. this doesn't typically matter anyways, because it would be super surprising if a tie get chosen to be in the MIS).


%\section{Handling of Ties}
%\label{sec:tie-handling}
%We treat each evaluation as a binary comparison between a winner and a loser, and discard any matchup that is annotated as a tie. 

%According to the original Chatbot Arena paper \citep{chiang2024chatbot}, ties are treated differently in different evaluation pipelines. For instance, the default leaderboard implementation by \citet{chiang2024chatbot} discards all ties before computing rankings using the Bradley--Terry model.

%Note, however, that in a \href{https://colab.research.google.com/drive/1KdwokPjirkTmpO_P1WByFNFiqxWQquwH#scrollTo=mSizG3Pzglte}{Chatbot Arena Leaderboard Calculation (Bradley-Terry model)} provided on the Chatbot Arena webpage, model rankings were computed using a weighted logistic regression. In this weighted version of the BT model, each pairwise comparison between two models $i$ and $j$ contributes a row to the BT estimation procedure. The weight attached to that row represents the number of times each pairwise comparison occurred. Within this weighted model, ties are treated evenly by splitting their weight equally across both directions.
